A Family of Exact Goodness-of-Fit Tests for High-Dimensional Discrete Distributions

The objective of goodness-of-fit testing is to assess whether a dataset of observations is likely to have been drawn from a candidate probability distribution. This paper presents a rank-based family of goodness-of-fit tests that is specialized to discrete distributions on high-dimensional domains. The test is readily implemented using a simulation-based, linear-time procedure. The testing procedure can be customized by the practitioner using knowledge of the underlying data domain. Unlike most existing test statistics, the proposed test statistic is distribution-free and its exact (non-asymptotic) sampling distribution is known in closed form. We establish consistency of the test against all alternatives by showing that the test statistic is distributed as a discrete uniform if and only if the samples were drawn from the candidate distribution. We illustrate its efficacy for assessing the sample quality of approximate sampling algorithms over combinatorially large spaces with intractable probabilities, including random partitions in Dirichlet process mixture models and random lattices in Ising models.

==> figures/tab-baselines.tex <==
%!TEX root=../main.tex

\begin{table*}[ht]
\centering
\scriptsize
\begin{tabular}{lllllll}
\toprule
Test Statistic
  & Data
  & Null Distribution
  & Critical Values
  & Equation
  & References
  \\
\midrule \\[-2ex]
Multinomial test
  & nominal
  & none
  & non-asymptotic
  & $\sum_{\tilde{O}<O}n!\prod_{x}\bp(x)^{\tilde{O}_x}/({\tilde{O}_x}!)$
  & \citep{horn1977} \\
Pearson chi-square
  & nominal
  & distribution-free
  & asymptotic
  & $\sum {(O_x-E_x)^2}/{E_x}$
  & \citep{pearson1900} \\
Likelihood ratio-test
  & nominal
  & distribution-free
  & asymptotic
  & $2\sum O_x\ln\left({O_x}/{E_x}\right)$
  & \citep{wilks1938}, \citep{williams1976} \\
Kolmogorov--Smirnov
  & nominal
  & distribution-dependent
  & non-asymptotic
  & $(1/2)\sum |O_x - E_x|$
  & \citep{hoeffding1965}, \citep{pettitt1977} \\
Cram\'er--von Mises
  & ordinal
  & distribution-dependent
  & asymptotic
  & $1/n\sum Z_x^2\bp(x)$
  & \citep{choulakian1994} \\
Watson
  & ordinal
  & distribution-dependent
  & asymptotic
  & $1/n\sum (Z_x-\bar{Z}_x)^2\bp(x)$
  & \citep{choulakian1994} \\
Anderson--Darling
  & ordinal
  & distribution-dependent
  & asymptotic
  & $1/n\sum Z_x^2\bp(x)/(H_x(1-H_x))$
  & \citep{choulakian1994} \\
Kolmogorov--Smirnov
  & ordinal
  & distribution-dependent
  & non-asymptotic
  & $\max_{s}|Z_x|$
  & \citep{conover1972}, \citep{pettitt1977} \\ \bottomrule
\end{tabular}
\caption{Common test statistics used for discrete goodness-of-fit testing in
low dimensions, where $n$ is the sample size; $x$ ranges over the values in
$\dom$; $O_x$ is the observed counts in cell $x$; $E_x \defas n\bp(x)$ is the
expected counts in cell $x$; $Z_x \defas \sum_{x' \le s}(O_{x'}-E_{x'})$;
$H_x \defas \sum_{x' \le x}E_{x'}$; and $\bar{Z} \defas \sum_{x' \le
x}Z_x\bp(x)$. While all these statistics are inappropriate for sparse data
and/or very large domains, they are listed here because several are
appropriate to use as subroutines when testing for uniformity of the proposed
stochastic rank statistic in Algorithm~\ref{alg:gof-uniform-rank} on a small
number of cells; see \citet{steele2006}.}
\label{tab:gof-baselines}
\end{table*}

